DiffDock-PP: Rigid Protein-Protein Docking with Diffusion Models

Understanding how proteins structurally interact is crucial to modern biology, with applications in drug discovery and protein design. Recent machine learning methods have formulated protein-small molecule docking as a generative problem with significant performance boosts over both traditional and deep learning baselines. In this work, we propose a similar approach for rigid protein-protein docking: DiffDock-PP is a diffusion generative model that learns to translate and rotate unbound protein structures into their bound conformations. We achieve state-of-the-art performance on DIPS with a median C-RMSD of 4.85, outperforming all considered baselines. Additionally, DiffDock-PP is faster than all search-based methods and generates reliable confidence estimates for its predictions. Our code is publicly available at $\texttt{https://github.com/ketatam/DiffDock-PP}$

==> tables/DB5_bound_NOT_finetuned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\centering
\caption{Complex prediction results on 25 samples from the DB5.5 test set (bound structures). NO finetuning on DB5.5}
\label{tab:db5_bound_not_finetuned}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  & \multicolumn{12}{c}{DB5-bound Test Set}                                                                           \\
                      & \multicolumn{6}{c|}{Complex RMSD (\AA)}  & \multicolumn{6}{c}{Interface RMSD (\AA)} \\ \cmidrule(l){2-13} 
Methods &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  Median &
  Mean &
  \multicolumn{1}{c|}{Std} &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  Median &
  Mean &
  Std \\ \midrule
EquiDock              & 0 & 4  & 8  & 17.00 & 16.00 & \multicolumn{1}{c|}{5.74} & 0     & 4      & 16    & 11.80    & 14.00    & 5.32     \\
DiffDock(40)          & 0 & 4  & 8  & 18.19 & 20.05 & \multicolumn{1}{c|}{8.88} & 0     & 0      & 8     & 19.30    & 21.78    & 10.45    \\
DiffDock(40) - oracle & 0 & 20 & 72 & 7.42  & 8.06  & \multicolumn{1}{c|}{3.44} & 0     & 20     & 80    & 7.53     & 7.57     & 2.92     \\ \bottomrule
\end{tabular}%
}


==> tables/DB5_bound_finetuned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\centering
\caption{Complex prediction results on 25 samples from the DB5.5 test set (bound structures). FINETUNED on DB5.5}
\label{tab:db5_test_finetuned}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{12}{c}{DB5-bound Test Set}                                                                             \\
                     & \multicolumn{6}{c|}{Complex RMSD (\AA)}    & \multicolumn{6}{c}{Interface RMSD (\AA)} \\ \cmidrule(l){2-13} 
Methods &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  Median &
  Mean &
  \multicolumn{1}{c|}{Std} &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  Median &
  Mean &
  Std \\ \midrule
Attract              & 44 & 44 & 52 & 9.55  & 10.09 & \multicolumn{1}{c|}{9.88}  & 44     & 44    & 52    & 7.48     & 10.69    & 10.90    \\
HDock                & 80 & 80 & 80 & 0.30  & 5.34  & \multicolumn{1}{c|}{12.04} & 80     & 80    & 80    & 0.24     & 4.76     & 10.83    \\
ClusPro              & 36 & 56 & 60 & 3.38  & 8.26  & \multicolumn{1}{c|}{7.92}  & 40     & 60    & 64    & 2.32     & 8.72     & 9.90     \\
PatchDock            & 4  & 4  & 16 & 18.26 & 18.00 & \multicolumn{1}{c|}{10.12} & 4      & 4     & 16    & 18.89    & 18.75    & 10.07    \\
EquiDock             & 0  & 0  & 16 & 14.14 & 14.73 & \multicolumn{1}{c|}{5.31}  & 0      & 0     & 16    & 11.97    & 13.23    & 4.93     \\
%DiffDock-S(40)       &    &    &    &       &       & \multicolumn{1}{c|}{}      &        &       &       &          &          &          \\
%DiffDock(10)         &    &    &    &       &       & \multicolumn{1}{c|}{}      &        &       &       &          &          &          \\
\ours(40)         &  12  &  12  & 24   &   14.07    &    -   & \multicolumn{1}{c|}{-}      &   8     &   12    &   24    &   15.12       &       -   &      -    \\ \bottomrule
\end{tabular}%
}


==> tables/DB5_unbound_NOT_finetuned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  & \multicolumn{8}{c}{DB5-unbound Test Set}                                                                          & \multicolumn{1}{l}{} \\
                      & \multicolumn{4}{c|}{Complex RMSD (\AA)} & \multicolumn{4}{c|}{Interface RMSD (\AA)} & Runtime (s)          \\ \cmidrule(l){2-10} 
Methods &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  \multicolumn{1}{c|}{Median} &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  \multicolumn{1}{c|}{Median} &
  Mean \\ \midrule
HDock                 & 0     & 0      & 16    & \multicolumn{1}{c|}{16.2}     & 0     & 0      & 12     & \multicolumn{1}{c|}{16.2}      & 615                  \\
EquiDock              & 0     & 0      & 8    & \multicolumn{1}{c|}{15.4}     & 0     & 0      & 44     & \multicolumn{1}{c|}{11.7}      & 5                    \\
%\ours{}(1)          & 0     & 1.6      & 9.6     & \multicolumn{1}{c|}{16.42}    & 0     & 0      & 12.8      & \multicolumn{1}{c|}{16.7}     &                      \\
\ours{}(40)          & 0     & 4      & 16     & \multicolumn{1}{c|}{14.61}    & 0     & 0      & 16      & \multicolumn{1}{c|}{15.58}     &                      \\ %\midrule
%\ours{}(40) - oracle & 0     & 16     & 56    & \multicolumn{1}{c|}{8.83}     & 0     & 12     & 56     & \multicolumn{1}{c|}{9.29}      &                      \\ 
\bottomrule
\end{tabular}%
}


==> tables/DIPS_test_set.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  & \multicolumn{8}{c}{DIPS Test Set}                                                     & \multicolumn{1}{l}{} \\
 &
  \multicolumn{4}{c|}{Complex RMSD (\AA)} &
  \multicolumn{4}{c|}{Interface RMSD (\AA)} &
  Runtime (s) \\ \cmidrule(l){2-10} 
Methods &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  \multicolumn{1}{c|}{Median} &
  \%\textless{}2 &
  \%\textless{}5 &
  \multicolumn{1}{l}{\%\textless{}10} &
  \multicolumn{1}{c|}{Median} &
  Mean \\ \midrule
\textsc{Attract}*               & 20 & 23 & 33 & \multicolumn{1}{c|}{17.17} & 20 & 22 & 38 & \multicolumn{1}{c|}{12.41} & 1285$^\dagger$                 \\
\textsc{HDock}*                 & \textbf{50} & \textbf{50} & 50 & \multicolumn{1}{c|}{6.23}  & \textbf{50} & 50 & 58 & \multicolumn{1}{c|}{\textbf{3.90}}  & 778$^\dagger$               \\
\textsc{ClusPro}*               & 12 & 27 & 35 & \multicolumn{1}{c|}{15.77} & 21 & 27 & 42 & \multicolumn{1}{c|}{12.54} & 10475$^\dagger$                 \\
\textsc{PatchDock}*             & 31 & 32 & 36 & \multicolumn{1}{c|}{15.25} & 32 & 32 & 42 & \multicolumn{1}{c|}{11.45} & 7378$^\dagger$                  \\
\textsc{AlphaFold-multimer}*              & 39  & 45  & 52 & \multicolumn{1}{c|}{8.61} & 45  & 47 & 58 & \multicolumn{1}{c|}{6.67} & 1560                    \\
\textsc{EquiDock}              & 0  & 8  & 29 & \multicolumn{1}{c|}{13.30} & 0  & 12 & 47 & \multicolumn{1}{c|}{10.19} & \textbf{3.88}                    \\
%\ours{}-S(40)        & 35 & 40 & 45 & \multicolumn{1}{c|}{12.34} & 37 & 40 & 50 & \multicolumn{1}{c|}{9.97}  &                      \\
%\ours{}(10)          & 31 & 40 & 46 & \multicolumn{1}{c|}{12.59} & 35 & 42 & 50 & \multicolumn{1}{c|}{10.04} &                      \\
\ours{}(1)          & 34 & 41 & 46 & \multicolumn{1}{c|}{11.95} & 36 & 42 & 53 & \multicolumn{1}{c|}{8.60} & 4.2                      \\
\ours{}(40)          & 42 & \textbf{50} & \textbf{55} & \multicolumn{1}{c|}{\textbf{4.85}} & 45 & \textbf{52} & \textbf{63} & \multicolumn{1}{c|}{4.23}  & 153                     \\ \midrule
\ours{}(40) - oracle & 71 & 79 & 86 & \multicolumn{1}{c|}{0.67}  & 72 & 82 & 91 & \multicolumn{1}{c|}{0.54}  & 153                      \\ \bottomrule
\end{tabular}%
}
